Emission-Line Galaxies from the Hubble Space Telescope Probing Evolution and Reionization Spectroscopically (PEARS) Grism Survey. II: The Complete Sample

We present a full analysis of the Probing Evolution And Reionization Spectroscopically (PEARS) slitess grism spectroscopic data obtained with the Advanced Camera for Surveys on HST. PEARS covers fields within both the Great Observatories Origins Deep Survey (GOODS) North and South fields, making it ideal as a random survey of galaxies, as well as the availability of a wide variety of ancillary observations to support the spectroscopic results. Using the PEARS data we are able to identify star forming galaxies within the redshift volume 0< z<1.5. Star forming regions in the PEARS survey are pinpointed independently of the host galaxy. This method allows us to detect the presence of multiple emission line regions (ELRs) within a single galaxy. 1162 Ha, [OIII] and/or [OII] emission lines have been identified in the PEARS sample of ~906 galaxies down to a limiting flux of ~1e-18 erg/s/cm^2. The ELRs have also been compared to the properties of the host galaxy, including morphology, luminosity, and mass. From this analysis we find three key results: 1) The computed line luminosities show evidence of a flattening in the luminosity function with increasing redshift; 2) The star forming systems show evidence of disturbed morphologies, with star formation occurring predominantly within one effective (half-light) radius. However, the morphologies show no correlation with host stellar mass; and 3) The number density of star forming galaxies with M_* > 1e9} M_sun decreases by an order of magnitude at z<0.5 relative to the number at 0.5<z<0.9 in support of the argument for galaxy downsizing.

==> table2s.tex <==
\begin{deluxetable}{ccccccrrrrcccc}
\tabletypesize{\footnotesize}
\setlength{\tabcolsep}{0.06in}
\tablewidth{0pt}

\tablecaption{Properties of PEARS Emission-Line Galaxies.\label{table2}}
\tablehead{
\colhead{PEARS} &
\colhead{PEARS}  &
\colhead{PEARS}  &
\colhead{R.A.}  &
\colhead{DEC} &
\colhead{Grism} &
\colhead{Flux} &
\colhead{Wavelength} &
\colhead{EW} &
\colhead{$i_{AB}$} &
\colhead{Line} &
\colhead{Line} \\
\colhead{Field} &
\colhead{ID}  &
\colhead{ELR ID}  &
\colhead{(deg)}  &
\colhead{(deg)} &
\colhead{Redshift} &
\colhead{($10^{-18}erg/s/cm^2$)} &
\colhead{(\AA)} &
\colhead{(\AA)} &
\colhead{(mag)} &
\colhead{ID} &
\colhead{Grade} \\
}
\rotate
\startdata
PEARS-N-1 & n30256 & 1  & 189.18592310 & 62.16982753 & 0.94 & $26.1 \pm 1.9$ &  7217 &   80 & 23.7 & \OII & 3.8\\
PEARS-N-1 & n30256 & 1  & 189.18592310 & 62.16982753 & 0.94 & $137.0 \pm 18.0$ &  9710 &  363 & 23.7 & \OIII & 3.1\\
PEARS-N-1 & n31345 & 1  & 189.16498516 & 62.17099244 & 0.49 & $39.8 \pm 12.1$ &  7437 &  194 & 26.1 & \OIII & 3.3\\
PEARS-N-1 & n33944 & 1  & 189.16105015 & 62.17608778 & 0.69 & $62.9 \pm 3.8$ &  8454 &  223 & 24.1 & \OIII & 3.7\\
PEARS-N-1 & n35090 & 1  & 189.20037133 & 62.17725706 & 0.65 & $26.0 \pm 2.4$ &  8237 &  212 & 24.4 & \OIII & 4.0\\
PEARS-N-1 & n35767 & 1  & 189.20747927 & 62.17882730 & 0.48 & $16.3 \pm 15.2$ &  7344 &  107 & 25.0 & \OIII & 3.0\\
\enddata
\tablecomments{This table is available in its entirety in the online journal. A portion of it is shown here.}

\end{deluxetable}

